MINER: A Hybrid Data-Driven Approach for REST API Fuzzing

In recent years, REST API fuzzing has emerged to explore errors on a cloud service. Its performance highly depends on the sequence construction and request generation. However, existing REST API fuzzers have trouble generating long sequences with well-constructed requests to trigger hard-to-reach states in a cloud service, which limits their performance of finding deep errors and security bugs. Further, they cannot find the specific errors caused by using undefined parameters during request generation. Therefore, in this paper, we propose a novel hybrid data-driven solution, named MINER, with three new designs working together to address the above limitations. First, MINER collects the valid sequences whose requests pass the cloud service's checking as the templates, and assigns more executions to long sequence templates. Second, to improve the generation quality of requests in a sequence template, MINER creatively leverages the state-of-the-art neural network model to predict key request parameters and provide them with appropriate parameter values. Third, MINER implements a new data-driven security rule checker to capture the new kind of errors caused by undefined parameters. We evaluate MINER against the state-of-the-art fuzzer RESTler on GitLab, Bugzilla, and WordPress via 11 REST APIs. The results demonstrate that the average pass rate of MINER is 23.42% higher than RESTler. MINER finds 97.54% more unique errors than RESTler on average and 142.86% more reproducible errors after manual analysis. We have reported all the newly found errors, and 7 of them have been confirmed as logic bugs by the corresponding vendors.

==> 12shepherd.tex <==


Dear shepherd, we have followed all the suggestions raised by the reviewers to revise the manuscript, which is denoted as "sec23summer-paper129-v2.pdf" in the attachment. We also provide the diff results to show the modifications, which can be found in the attachment. In the following, we mainly introduce our modification content to each suggestion in Comment A1. 

1. The presentation needs to accurately reflect the improvement over prior work (both qualitative and quantitative) without over-claiming. Particularly, refer to Rev-D and your response to it.

Response: In the revised manuscript, we first change the expression of the improvement ratio from "0.33X" to "33.00%". Then, we report more average results in the revised manuscript, in order to show the overall performance comparison without over-claiming. For instance, we mainly use the average pass rate to measure the performance of three fuzzers on page 9. Finally, we carefully check all the analysis results to prevent clerical errors. 

2. The extrinsic evaluation needs to be expanded to the other 2 cloud services.

Response: We follow the comments from Rev-D and extend real error analysis to Bugzilla and WordPress. For instance, our fuzzers find a new security bug on WordPress, which RESTler misses. More details can be found in the manuscript. 

3. Address all of the presentation-related comments from Rev-A and Rev-E. Particularly, a. Integrate examples to explain the design, b. Fill in the gaps in the description of the evaluation. c. Provide formal key definitions early on. d. Reduce repetition where unnecessary (particularly if it helps with saving space). c. Clearly state the limitations of the work. 

Response: We follow the comments from all the reviewers to improve the presentation. Specifically, we provide an example to convert the web description of a request to a request template as shown in Fig. 1 in the manuscript; We add examples to help understand most places that contain key concepts; We carefully revise the description of Section 4 (Evaluation) and Section 5 (Further Analysis) based on the reviewers' comments; We follow the comments to provide key definitions early on. For instance, we explain how a cloud service behaves with an example of a delete request on page 1 in the revised manuscript; We revise the entire manuscript to fit the 18-page requirement; We follow the comments to improve the description of the limitations of the work, e.g., the limitations of existing approaches and error reproduction. 

4. Explain what is security-specific about MINER, early on. If the tool is broader (i.e., can detect security and non-security work), and if prior work in fuzzing in security venues is along the same lines, describe how MINER builds upon such prior work, again early in the paper. 

Response: In the revised manuscript, we first introduce on page 1 that most security bugs, like use-after-free bugs that can lead to private data leakage, require long sequences to be triggered as shown in "Checking Security Properties of Cloud Service REST APIs". The underlying reason is that security bugs often require complex execution logic to trigger. Then, we introduce the limitations of existing REST API fuzzers in the sequence construction and request generation, which are two main problems for REST API fuzzers as introduced on page 1. To overcome these limitations, we propose MINER, which implements different designs to improve the sequence construction and request generation. In the evaluation, our designs help MINER find 5 new security bugs that access deleted resources. On the contrary, RESTler cannot find any of them. The results demonstrate that MINER is efficient at finding security bugs and our designs contribute to security bug discovery. 

Furthermore, to improve the readability, we revise the fuzzer name from "MINER" and "MINER_PLUS" to "MINER_PART" and "MINER", as the old "MINER_PLUS" is the complete prototype which contains all 3 designs. We also revise the key concepts from "<parameter, value> pairs"  and "parameter combinations"  to "param-value pairs" and "param-value lists". We follow the comments of Rev-A to revise the bibliography. 

If you have any suggestions, please let us know. 
